Vehicle Reconstruction and Texture Estimation Using Deep Implicit Semantic Template Mapping

We introduce VERTEX, an effective solution to recover 3D shape and intrinsic texture of vehicles from uncalibrated monocular input in real-world street environments. To fully utilize the template prior of vehicles, we propose a novel geometry and texture joint representation, based on implicit semantic template mapping. Compared to existing representations which infer 3D texture distribution, our method explicitly constrains the texture distribution on the 2D surface of the template as well as avoids limitations of fixed resolution and topology. Moreover, by fusing the global and local features together, our approach is capable to generate consistent and detailed texture in both visible and invisible areas. We also contribute a new synthetic dataset containing 830 elaborate textured car models labeled with sparse key points and rendered using Physically Based Rendering (PBRT) system with measured HDRI skymaps to obtain highly realistic images. Experiments demonstrate the superior performance of our approach on both testing dataset and in-the-wild images. Furthermore, the presented technique enables additional applications such as 3D vehicle texture transfer and material identification.

==> sections/2_related_bk.tex <==
\begin{figure*}
\begin{center}
\includegraphics[scale=0.27]{pipeline2.png}
\end{center}
\caption{The overview of our approach. Given the input monocular RGB-Mask, vehicle digitization is achieved by geometry and texture reconstruction. We first convert the original picture into an albedo map, and then extract multi embedding latent codes with ResNet-based encoders in Latent Embedding. Conditioned on these latent codes, our neural networks can infer SDF to reconstruct mesh surface and then regress RGB value for surface points.}
\label{fig:pipeline}
\end{figure*}

%------------------------------------------------------------------------
\section{Related Work}
\label{sec:related}


%-------------------------------------------------------------------------
\subsection{Monocular Vehicle Reconstruction}
%In this section, we mainly focus on monocular vision based vehicle shape-texture reconstruction. 

With large-scale synthetic datasets such as ShapeNet~\cite{Chang2015ShapeNet}, many works~\cite{Oechsle2019Texture,sun2018im2avatar,3D-R2N2} have allowed deep neural networks to be trained on the task of vehicle reconstruction from single images. By combining with shape reconstruction methods like~\cite{Mescheder2019Occupancy,Park2019DeepSDF}, Texture Field can generate plausible textured vehicle model from single images based on implicit representation. Im2Avatar~\cite{sun2018im2avatar} can achieve colorful 3D reconstruction by decomposing shape and color learning into two different procedures in a 3D voxel representation. Although these methods can achieve impressive results in synthetic dataset, they are incompetent at challenging real-world traffic scenarios due to the domain gap.

In the field of autonomous driving, works focusing on shape recovery and pose estimation~\cite{Kundu_2018_CVPR_3DRCNN,Song_2019_CVPR_ApolloCar3D,Manhardt2018ROI,Zakharov2020Autolabeling,Ku_2019_CVPR_Monocular3DObjectDetection,Grabner_2018_CVPR_3DPoseEstimation,Chabot_2017_CVPR_DeepManta,Mottaghi_2015_CVPR_ACoarse2Fine} can naively expand to texture reconstruction with projective texturing. However, direct unprojection can only obtain the texture of visible parts and is incapable of recovering consistent 3D texture. 
% For example, ROI-10D[] proposed a monocular deep network that can lift 2D detections in 3D for metrically pose estimation and shape recovery. 

Recently, many works~\cite{beker2020monocularDifferentiableRendering,Henderson2020Leveraging,Kanazawa_2018_ECCV_Learning_Category-Specific,Learning_single-image_3D_reconstruction, Gadelha20183DShapeInduction} concentrate on vehicle 3D texture recovery under real environments. Due to the lack of ground truth 3D data of real scene, they mainly pay attention to reconstruct 3D models from 2D data utilizing unsupervised or self-supervised learning.  \cite{beker2020monocularDifferentiableRendering}  presented a self-supervised approach based on differentiable rendering for 3D shape reconstruction and localization of rigid objects from monocular images. \cite{Henderson2020Leveraging} propose a self-supervised approach that allows learning from collections of 2D images without any 3D information and a new generation process for 3D meshes that guarantees no self-intersections arise. \cite{Gadelha20183DShapeInduction} designs PrGANs which can infer the underlying 3D shape distribution without using any 3D, viewpoint information, or annotation. \cite{Learning_single-image_3D_reconstruction} learns to generate and reconstruct concave object classes under known lighting. Though these works successfully get rid of dependencies of 3D annotations and generate meaningful vehicle textured models, they still suffer from following shortcomings: 
1) reconstruction of shape and texture is coarse and over-smooth;
2) mostly rely on the approximately uniform light conditions, which is hard to meet in real street scene;
3) texture representation is built on rigid texture parameterizations.
In contrast, our method avoids cumbersome manual design and is not restricted by the limited resolution or fixed topology. With effective representation and novel feature extraction strategy, our method can recover fine vehicle model under challenging environments.

In addition, some works~\cite{VON,Novel_Views_of_Objects, View_synthesis_by_appearance_flow, 2017Transformation} focus on novel view synthesis, which infer texture in 2D domain. Although these works can produce realistic images, they are lack of compact 3D representation, which is not in line with our goal.



%-------------------------------------------------------------------------
\subsection{Deep Implicit representation}
Traditionally, implicit functions represent shapes by constructing a continuous volumetric field and embedding meshes as its iso-surface~\cite{Carr2001Reconstruction,GREG2002Modelling,2004Interpolating}. In recent years, implicit functions have been implemented with neural networks ~\cite{Park2019DeepSDF,Mescheder2019Occupancy,Chen2019Learning,Gropp2020Implicit,2019DISN,2020PIFu,Jiang2020Local, Chabra2020Deep, Hao2020DualSDF} and have shown promising results. For example, DeepSDF~\cite{Park2019DeepSDF} proposed to learn an implicit function where the network output represents the signed distance of the point to its nearest surface. Other approaches defined the implicit functions as 3D occupancy probability functions and turned shape representation into a point classification problem~\cite{Mescheder2019Occupancy,Chen2019Learning,2019DISN,2020PIFu}. Some latest studies proposed to blend multiple local implicit functions in order to capture more geometric details~\cite{Jiang2020Local, Chabra2020Deep}. DualSDF~\cite{Hao2020DualSDF} extended DeepSDF by introducing a coarse layer to support shape manipulation. DIT~\cite{Zheng2021DIT} extended DeepSDF by embedding a template to reason dense correspondences between different shapes. 

As for texture inference, following this path, both Texture Fields~\cite{Oechsle2019Texture} as well as PIFu~\cite{2020PIFu} defines textures implicitly as a function of 3D position. The former uses global latent codes separately extracted from input image and geometry whereas the latter leverages local features pixel-aligned with input image. Compared with the above implicit-function-based texture reconstruction approaches~\cite{2020PIFu,Oechsle2019Texture} which predict texture distribution in the whole 3D domain, our method explicitly constrains the texture distribution on the 2D surface of the template model with deep implicit semantic template representation, implemented by geo-tex joint training strategy. Furthermore, we utilize both global and local feature embedding to enhance details as well as keep consistency. 
%Experiments in Sec.~\ref{sec:experiments} show convincing comparison results and demonstrate that our representation is more suitable for vehicle digitization.

==> sections/3_overview_bk.tex <==
\begin{figure*}
\begin{center}
\includegraphics[scale=0.30]{pipeline2.png}
\end{center}
\caption{The overview of our approach}
\label{fig:pipeline}
\end{figure*}


%-------------------------------------------------------------------------
\section{Overview}

In this section, we would first introduce our overall idea and explain why our proposed DIST representation is more suitable for vehicle 3D texture reconstruction compared with previous implicit-function based representation TF[]. Then we would introduce the overview over our method is shown in Fig\ref{fig:pipeline}.

%-------------------------------------------------------------------------
\subsection{Problem Formulation and Analysis}

The appearance of an object observed in pictures is generated by the projection of real-world high-dimensional physics in the low-dimensional camera plane. The process of recovering the intrinsic components of the object itself from observation is known as "inverse rendering." Though inverse rendering on 2D image field has made great advances, this only focus on visible area in 3D space. As for the problem on monocular image based 3D intrinsic texture reconstruction, we can formulate the color recovery of one specific surface point as the following Inverse Rendering function $\mathcal{F}$ :
\begin{equation}
c=\mathcal{F}(p,m,I,L,S,C) \label{eq1}
\end{equation}
where $p\in{R^3}$ is the surface point 3D position, $c\in{R^3}$ is the corresponding recovered color value, $m\in{R^m}$ is the corresponding material parameters on the $p$, $I\in{R^I}$ is the appearance information from observed image. $L\in{R^L}$ represents effects of environment lighting condition, $S\in{R^S}$ represents effects of object shape geometry (e.g. occlusion, surface normal), $C\in{R^C}$ represent camera-related parameters. Total sum of all variable dimensions is $3+R^m+R^I+R^L+R^S+R^C$. Since it is impossible to learn the decomposition without any constraints on the intrinsic components,  in order to better inference albedo texture, it's essential to introduce some prior knowledge  or combine some of above  physics information to filter out other nuisance variables.  

Based on the idea of implicit function, Texture Fields representation defines the surface texture as a continuous function by means of a 3D vector field $\mathcal{F}:R^3\rightarrow{R^3}$, which maps a 3D point $p$ to the rgb value $c$, where $F$ is the function approximated using a deep neural network. In practice, in order to represent diverse texture on multiple object instances using one network, TF is conditioned on the additional input 2D image and 3D CAD model and thus the function F can be written as : 
\begin{equation}
c=\mathcal{F}(p,I,S): p\in{R^3}, I\in{R^I}, S\in{R^S}\label{eq2}
\end{equation}
TF uses two high-dimensional embedding vectors $t$ and $s$ separately encoded from the 2D image and 3D models to represent appearance and geometry information. With 3D Texture represented by $\mathcal{F}$, textured mesh can be obtained by concatenating all surface sample points $p$ with embedding $t$ and $s$ as input. 

In contrast to TF, with a template car model as intermediary, our method separates the process of 3D texture reconstruction into two steps and infers texture distribution on the surface of the template model. As for our RGB mapping process,  all input sample points $p$ are restricted on the template’s surface hence indeed share only two-degree-of-freedom. The input shape is constant as template geometry. Besides, as the material parameters corresponding to a specific surface point of template car is fixed (in fact, the class of vehicles mostly share similar material in same  corresponding parts), the variable $m$ can be totally expressed by the surface point location p(e.g. a lookup table). With all these advantages and priors, the Inverse Render function of our method of can be written as :
\begin{equation}
c=\mathcal{F}(p_{tp}, I): p_{tp}\in{R^2}, I\in{R^I}\label{eq3}
\end{equation}
Compared with Eq\ref{eq2} of TF method, which use total $3$+$R^I$+$R^S$ dimensional variables, our method uses only $2$+$R^I$ dimensional parameters to represent $3$+$R^I$+$R^m$+$R^S$ dimensional variables’ information.

\textbf{Conclusion:} Aiming at vehicle 3D texture recovery, our method can be more expressive with less complexity.

Based on the above analysis, such encouraging aforementioned conclusions relies on our proposed assumption that we can constrain the texture distribution on the 2D surface of template model. We achieve this goal with the process of semantic template mapping, which can be formulated as :
\begin{equation}
p_{tp}=\mathcal{W}(p_{tp}, S)\label{eq4}
\end{equation}
where $\mathcal{W}:R^3*R^S\rightarrow{R^3}$ is a spatial warping function mapping the 3D point p to the corresponding location $p_{tp}$ in template field conditioned on the shape variable $S$. To represent and reconstruct geometry, similar to [zerong], an additional implicit function  $\mathcal{T}:R^3\rightarrow{R^1}$ to query the signed distance value at $p_{tp}$, and the surface is defined as the zero-level set of $\mathcal{T}$ and can be extracted using Marching Cube[].


\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.40]{template_mapping.png}
\end{center}
   \caption{Visulize of uvw mapping and semantic mapping}
\label{fig:uvw_mapping}
\end{figure}

%-------------------------------------------------------------------------
\subsection{Main PipeLine}
Based on uncalibrated monocular input, our goal is to reconstruct the underlying 3D geometry and texture of a car. Fig 2 illustrates the overview of our network. The pipeline starts with a monocular image and corresponding 2D instance mask detections, which can be produced by off-the-shelf 2D detectors~\cite{2017Mask}. Firstly, we infer the intrinsic color in 2D image field by means of image2image translation, and the recovered albedo image will be used as another input. Then, as shown in the figure, our network consists of three parts, i.e., latent embedding, geometry reconstruction and texture estimation.

Similar to other implicit functions based methods, we use latent codes extracted from images to condition implicit function network blocks. In the latent embedding, from 4-dim input (rgbm) multi ResNet-based~\cite{2016Deep} encoders are used to separately embed shape, pose, global and local texture information as $Z_{shape}$, $Z_{pose}$, $Z_{tex}$ and $Z_{loc\_tex}$. Specifically, predicted albedo image is fed into texture encoders to extract de-illuminated texture latent codes. For geometry reconstruction, volume samples are sequentially input to the template mapping block and template sdf decoder to predict the continuous signed distance field. For texture estimation, surface points on reconstructed mesh are firstly warped to the template surface conditioned on $Z_{shape}$, and then pass the RGB decoder to predict texture distribution. Practically, the variable $I$ representing the appearance information from observed image in Eq\label{eq3} is the fusion of pose latent code $Z_{pose}$, global texture feature $Z_{tex}$ and local texture feature $Z_{loc\_tex}$. Resulting from the great pose diversity in vehicle images, we explicitly separate $Z_{pose}$ and do not wish texture encoders to have to account for this variability. The shape latent code $Z_{shape}$ to be concatenated with 3D point p represent variable S in Eq\label{eq4}. .Hence Eq\label{eq4}. and Eq\label{eq3}. can be rewritten as:

\begin{equation}
p_{tp}=\mathcal{W}(p, Z_{shape})\label{eq5}
\end{equation}
\begin{equation}
c=\mathcal{F}(p_{tp},Z_{shape},Z_{pose},Z_{tex},Z_{loc\_tex})\label{eq6}
\end{equation}



==> sections/4_method_bk.tex <==


\begin{figure*}
\begin{center}
\includegraphics[scale=0.20]{end2end_architecture.png}
\end{center}
\caption{End-to-end training Network}
\label{fig:train_pipe}
\end{figure*}

%-------------------------------------------------------------------------
\section{Method}
\subsection{Dataset Generation}
To generate synthetic dataset, we use 83 various industry-grade 3D CAD models covering common vehicle types, of which 63 are used in train-dataset and the other 20 are used to test. Each model is labeled with 23 semantic key points defined as shown in Fig. We specifically select a commonly seen car as a template. To enrich the texture and orientation diversity of our dataset, we assign ten different texture for each models and each textured mesh is randomly rotated around yaw axis. In order to narrow the domain gap between our synthetic dataset with real scene, we render the realistic image using Physically Based Rendering (PBRT)[] system with real sky map in the Laval HDR Sky Database~\cite{Laval_HDR_sky}. To simulate the observe view in real street environment, car models are randomly set in different 3D position and rendered in high-resolution (2048*1024) and wide angle ($Fov=50^{\circ}$) image. After car instances are cropped using its correspondence instance masks, all cropped images are resized and centered in images with the resolution of 256*256, together with corresponding front and back depth and albedo maps. Finally, we get a training set with 6300 images and a testing set with 2000 images in total.

As for the supervision for geometry reconstruction, after normalizing car cads to a unit sphere, we refer to data preparation method in Onet~\cite{Mescheder2019Occupancy}to generate watertight meshes and follow the sampling strategy in DeepSDF~\cite{Park2019DeepSDF} to obtain spatial points with their calculated SDF value.


%-------------------------------------------------------------------------
\subsection{Training}
This sections describes how we train our network end-to-end to implement implicit semantic template mapping. See Fig\ref{fig:train_pipe} for a visual illustration. 
The backbone of VERTEX is composed of three main network blocks: Template Mapping, Template Sdf Decoder, and RGB Decoder, which are continuous implicit mapping functions represented by multi-layer perceptions(MLPs). As the figure shows, from the template mapping block, two branches separately lead to reconstruction of geometry and texture estimation. 
For geometry reconstruction, we mainly train by minimizing the $\mathcal{l}$1-loss between the predicted sdf value and the groud-truth:

\begin{equation}
    L_{geo}=\frac{1}{N_{sdf}}\sum_{i=1}^{N_{sdf}}\left \| \mathcal{T}(\mathcal{W}\left ( p_i, Z_{shape} \right ))-s_i  \right \|_1 \label{eq7}
\end{equation}
where $N_{sdf}$ represents the number of input sample points, $Z_{shape}$ is the shape latent code corresponding to the volume sample point $p_i$, and $s_i$ is the corresponding ground truth SDF value on the $p_i$. Additionally, to accelerate convergence, benefiting from the disentangled template representation, we can train Template SDF Decoder directly using the sample points of template car CAD without any latent code:
\begin{equation}
    L_{tp\_sdf}=\frac{1}{N_{tp\_sdf}}\sum_{i=1}^{N_{tp\_sdf}}\left \| \mathcal{T}(p_i)-s_i  \right \|_1 \label{eq8}
\end{equation}
where $p_i$ represents the volume sample point around template model and $s_i$ is the corresponding SDF value.

For texture estimation, we mainly train by minimizing the l1-loss between the regressed RGB value and the ground-truth:
\begin{equation}
    L_{tex}=\frac{1}{N_{sf}}\sum_{i=1}^{N_{sf}}\left \| \mathcal{F}(\mathcal{W}\left ( p_i, Z_{shape} \right ), Z_{pose},  \mathcal{f}(Z_{tex}, Z_{loc\_tex}))-c_i  \right \|_1 \label{eq9}
\end{equation}
where $N_{sf}$ represents the number of input surface points, $c_i$ is the corresponding ground truth color value on the surface point $p_i$, $Z_{shape}$, $Z_{tex}$, $Z_{loc\_tex}$ and $Z_{pose}$ are latent codes corresponding to the $p_i$, of which $Z_{loc\_tex}$ is sampled according to the 2D projection of pi on the feature maps. $\mathcal{f}$ is a simple function represented by MLP to fuse global and local texture latent codes. 

In specific implementations, inspired by recent work [] using Fourier encoding, to balance the dimension of latent codes and points 3D positon input to $\mathcal{F}$, we apply a simple linear layer to mapping $p_{tp}$ to high-dimensional vectors, which can obviously accelerate the convergence during training.

As for $Z_{pose}$, as 3D rotations of most vehicle in street view are mainly focus on the rotation of the yaw axis, we simply represent the pose information with the egocentric orientation~\cite{}[3DRCNN] of the yaw axis. To supervise the pose encoder, instead of directly regress 1D parameter, we use 2D sin-cos-encoding vector according with the periodicity of rotation.
\begin{equation}
    L_{pose}=\left \| o - o^* \right \|_1 \label{eq10}
\end{equation}
where $o$ is the sin-cos-encoding of the orientation and $o^{*}$ present the corresponding ground truth. $Z_{pose}$ is generated by upgrading the dimension of o with simple MLP.

Instead of the training schedule of geometry before texture, we simultaneously minimize $L_{tex}$\label{eq9} and $L_{geo}$\label{eq7}, using the consistency between RGB color and semantic parts to guide the template mapping to be semantic-preserving. Besides, concentrating on Template Mapping block, key points pair between instance vehicle and template model are used as weak supervision to calculate loss term:
\begin{equation}
    L_{kps}=\frac{1}{N_{kps}}\sum_{i=1}^{N_{kps}}\left \| \mathcal{W}\left (k_i, Z_{shape} \right ) -k_i^*  \right \|_1 \label{eq11}
\end{equation}
where $N_{kps}$ represents the number of input key points, $k_i$ and $k_i^*$ are the corresponding keypoints on instance and template.

The total loss function is formulated as the weighted sum of above mentioned term:
\begin{equation}
    L = L_{tex} + w_p*L_{pose}+w_k*L_{kps}+w_{g}*L_{geo}+w_{g}*L_{tp\_sdf}
    \label{eq13}
\end{equation}
With embedding latent codes implicitly depending on the parameters of encoders, the whole network is trained end-to-end by minimizing Eq\label{eq13}.

However, we found that jointly training $Z_{tex}$ and $Z_{loc\_tex}$ suffers from overfitting. The problem is that it’s much easier for $Z_{loc\_tex}$ to converge than $Z_{tex}$ causing the recovered texture to rely on $Z_{loc\_tex}$ and $Z_{tex}$ ineffectual, which is harmful to generate robust and consistent texture estimation. Hence, practically we first input $Z_{tex}$ alone as texture representation by setting $Z_{loc\_tex}$ as all-zero vectors, and $Z_{loc\_tex}$ is incorporated into training after basic convergence.

As for the problem of recovering texture in the intrinsic domain, we have tried to extract texture latent codes directly from the input image, and ask RGB Decoder to learn to remove complex lighting effects. However such solution worsen the accuracy of texture estimation and lead to over-smooth results. Considering the good performance of image-to-image translation networks in the 2D field, we train a Unet based network to produce albedo image.

%-------------------------------------------------------------------------
\subsection{Inference}

As shown in the pipeline in Fig\ref{fig:pipeline}, during inference, we first regress signed distance field following the branch of Template reconstruction, and then 3D points on the surface extracted are input to the branch of Texture Estimation to recover surface texture. However, because of the lack of ground truth camera intrinsic and extrinsic parameters, it is difficult for 3D point $p$ to sample the corresponding local feature from feature map to use as $Z_{loc\_tex}$, which poses a significant challenge. We address the problem by setting a virtual camera and optimize 6D pose under render-and-compare optimization framework.


We assume that the observed image is the central projection of normalized model related to a virtual perspective camera with a narrow FOV of $Fov=10^{\circ}$. 3D rotation is initialized with the egocentric orientation output from pose encoder and initial distance is set as 10m. We use the publicly available differentiable renderer from ~\cite{kato2018neural}. Fixing the model scale, we can optimize virtual 6D pose by minimizing 2D silhouette loss and establish projective correspondences between 3D surface points and feature maps. 


